An updated survey of Active Galaxies with the HAWC gamma-ray observatory

We present an update of the survey of Active Galaxies with the High Altitude Water Cherenkov (HAWC) gamma-ray observatory. This work adds 567 days of HAWC data to the previously published survey, providing a refined analysis of an updated total exposure of 2090 days. The sample includes 138 nearby AGNs from the 3FHL catalog. We fit a modified power-law to their very high energy spectra, including the exponential attenuation caused by the Extragalactic Background Light. We found four sources with significant detections (above 5$\sigma$): the radio galaxy M87 and the BL Lac objects Mkn 421, Mkn 501 and 1ES 1215+303. We also report eight sources with a marginal detection (between 3$\sigma$ and 5$\sigma$) of which seven are classified as BL Lac objects and one as a radio galaxy.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

